DDMI: Domain-Agnostic Latent Diffusion Models for Synthesizing High-Quality Implicit Neural Representations

Recent studies have introduced a new class of generative models for synthesizing implicit neural representations (INRs) that capture arbitrary continuous signals in various domains. These models opened the door for domain-agnostic generative models, but they often fail to achieve high-quality generation. We observed that the existing methods generate the weights of neural networks to parameterize INRs and evaluate the network with fixed positional embeddings (PEs). Arguably, this architecture limits the expressive power of generative models and results in low-quality INR generation. To address this limitation, we propose Domain-agnostic Latent Diffusion Model for INRs (DDMI) that generates adaptive positional embeddings instead of neural networks' weights. Specifically, we develop a Discrete-to-continuous space Variational AutoEncoder (D2C-VAE), which seamlessly connects discrete data and the continuous signal functions in the shared latent space. Additionally, we introduce a novel conditioning mechanism for evaluating INRs with the hierarchically decomposed PEs to further enhance expressive power. Extensive experiments across four modalities, e.g., 2D images, 3D shapes, Neural Radiance Fields, and videos, with seven benchmark datasets, demonstrate the versatility of DDMI and its superior performance compared to the existing INR generative models.

==> Figure/arbitrary_image.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.94\textwidth]{./Figure/arbitrary_image.pdf}
    \caption{\textbf{Arbitrary-scale INR generation}. We present the generation results of arbitrary-scale INR generation for images with a single model: zoom-in (upper-row) and arbitrary-resolution generation (bottom-row). INR-LDM can generate consistent, high-quality images over multiple scales.}
    \label{fig:main_qualitative}
\end{figure}

==> Table/main_plus_table_figure.tex <==
\begin{table}[ht]
\centering
\begin{minipage}{0.45\linewidth}
\centering
\includegraphics[width=0.95\linewidth]{Figure/analysis_decomposition.png}
    \captionof{figure}{\textbf{HDPE analysis.} %The upper two rows show generated images whereas the bottom one shows the spectral magnitude after applying Fourier transform. The far left column indicates the generated image. Other columns indicate the generated image with (a): $\mathbf{p}^2, \mathbf{p}^3$, (b): $\mathbf{p}^1, \mathbf{p}^3$, and (c): $\mathbf{p}^1, \mathbf{p}^2$ zeroed out, respectively. We employ histogram equalization for better visualization.
    }
\end{minipage}%
%\hspace{4mm}
\begin{minipage}{0.48\linewidth}
\caption{FID results on AFHQv2 Dog.}
\resizebox{0.96\linewidth}{!}{%
\begin{tabular}{lccc} 
\hline
              & Acc $\uparrow$           & CLIP-S $\uparrow$        & TMD $\downarrow$            \\ 
\hline
\hline
IMLE~\cite{liu2022towards}          & 34.79          & -              & 0.891           \\
Auto-SDF~\cite{mittal2022autosdf}      & 83.88          & -              & 0.581           \\
Diffusion-SDF~\cite{li2023diffusion} & 88.56          & 28.63          & \textbf{0.169}  \\
\hline
\textbf{DALM (Ours, $w=3$)}          & \textbf{91.30} & \textbf{30.30} & 0.204          \\
\hline
\end{tabular}
\label{tab:t2s}
}
%\vspace{5mm}
\caption{Ablation study.}
\centering
\resizebox{0.96\linewidth}{!}{%
\begin{tabular}{ccc|cc} 
\hline
\begin{tabular}[c]{@{}c@{}}Latent \\type\end{tabular} & HDPE & CFC & \begin{tabular}[c]{@{}c@{}}First Stage\\(PSNR)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Second Stage\\(FID)\end{tabular}  \\ 
\hline
1d                                                    &      &     & 30.24                                                           & -                                                            \\
2d                                                    &      &     & 32.72                                                       & 8.54                                                         \\
2d                                                    &    \checkmark   &     & 33.17                                                       & 8.23                                                         \\
2d                                                    &   \checkmark    &  \checkmark    & 33.56                                                       & 7.82         \\                      
\hline
\end{tabular}
}
\end{minipage}
\end{table}
